Submodular Secretary Problem with Shortlists

In submodular $k$-secretary problem, the goal is to select $k$ items in a randomly ordered input so as to maximize the expected value of a given monotone submodular function on the set of selected items. In this paper, we introduce a relaxation of this problem, which we refer to as submodular $k$-secretary problem with shortlists. In the proposed problem setting, the algorithm is allowed to choose more than $k$ items as part of a shortlist. Then, after seeing the entire input, the algorithm can choose a subset of size $k$ from the bigger set of items in the shortlist. We are interested in understanding to what extent this relaxation can improve the achievable competitive ratio for the submodular $k$-secretary problem. In particular, using an $O(k)$ shortlist, can an online algorithm achieve a competitive ratio close to the best achievable online approximation factor for this problem? We answer this question affirmatively by giving a polynomial time algorithm that achieves a $1-1/e-\epsilon -O(k^{-1})$ competitive ratio for any constant $\epsilon > 0$, using a shortlist of size $\eta_\epsilon(k) = O(k)$. Also, for the special case of m-submodular functions, we demonstrate an algorithm that achieves a $1-\epsilon$ competitive ratio for any constant $\epsilon > 0$, using an $O(1)$ shortlist. Finally, we show that our algorithm can be implemented in the streaming setting using a memory buffer of size $\eta_\epsilon(k) = O(k)$ to achieve a $1 - 1/e - \epsilon-O(k^{-1})$ approximation for submodular function maximization in the random order streaming model. This substantially improves upon the previously best known approximation factor of $1/2 + 8 \times 10^{-14}$ [Norouzi-Fard et al. 2018] that used a memory buffer of size $O(k \log k)$.

==> Impossiblesave.tex <==
%\section{Impossibility Result}

In this section we provide an upper bound showing the following:

\hardness*

%\begin{theorem}
%There is no algorithm achieving asymptotic competitive ratio $7/8+\epsilon$ for submodular secretary problem using $o(n)$ selections. 
%\end{theorem}

%\mcomment{In the following proof we will consider a submodular $k+1$-secretary} problem. 
In the following proof, for simplicity of notation, we prove the desired bound for submodular $k+1$-secretary problem. %Since $k+1=O(k)$, the upper bound derived will imply the stated bound for the  submodular $k$-secretary problem. 
First, we define a monotone submodular function $f$ as follows. 
For $n>0$, the ground set consists of two types of elements, $A$ and  $B$, such that
$f(a)=k$ for $a\in A$ and $f(b)=1$ for $b\in B$. %There are infinitely many elements of $A$ and $B$. 
\scomment{Don't you just need $L$ items of type $A$ and $n-1$ items of type $B$?}
There are $L:=n/2k$ items of type $A$ and
$n-1$ items of type $B$.
Also there is a collection of {\it disjoint} sets $T_{\ell}=\{a_1^{\ell}, b_1^{\ell},\cdots, b^{\ell}_{k}\}$, $\ell=1,2, \ldots L$, such that $a_1^{\ell}\in A$ and $b_j^{\ell}\in B$, and $f(T_{\ell})=2k$.
\scomment{infinite number of such sets? or will $L$ suffice?} 
\mcomment{in the definition of function it should be infinite but in the input we use $n/2k$ of them}
\scomment{After going through the proof, I don't see why you need infinite number, it seems just $L=n/2k$ will suffice. Where are you using that there are infinte number of $T^\ell$?}
\mcomment{
The reason is that you should give one functions $f$ that works for all $n$. Otherwise one may claim that for any given function $f$ there is large enough $N_f$ so that we can go beyond 7/8, for $n>N_f$. 
}

Now define 
$$g(t):=k+k/2+\cdots+ (t-ik)/2^i$$
where $i=\floor{t/k}$. It is easy to see that $g$ is a monotone submodular function.
Now define $f$ as follows:
\begin{itemize}
\item $|S\cap A| \ge 2 \implies f(S):=2k+1$
\item $|S\cap A|=0 \implies f(S):=1+g(|S|-1)$
\item $|S\cap A|=1 :$
\begin{itemize}
\item $S\cap A\notin\{a^{\ell}_1\}_{\ell>0} \implies f(S):=k+\frac{1}{2} g(|S|-1)$
\item $S\cap A= \{a_1^{\ell}\}$ for some $\ell$  $\implies f(S):=\min\{2k+1, k+\frac{1}{2} g(|S|-1)+k'/2^{i+1}\}$, where $k'=|S\cap\{b^{\ell}_1,\cdots, b_k^{\ell}\} |$.
\end{itemize}
\end{itemize}
Note that for any subset $S$, $f(S)\le 2k+1$.
\begin{lemma}
$f$ is a monotone submodular function.
\end{lemma}
\begin{proof}
We have to show that for elements $x$ and subsets $S\subseteq T$, $\Delta_f(x|S) \ge \Delta_f(x|T)$.
We consider the following cases:
\begin{itemize}
\item if $|T\cap A| \ge 2 \implies f_T(x)=0$, so it is trivial.
\item if $|T\cap A| =0 \implies |S\cap A|=0 \implies \Delta_f(x|S) \ge \Delta_f(x|T)$ because of submodularity of $g$.
\item if $|T\cap A|=1 \implies |S\cap A|\le 1$
\begin{itemize}
\item if $|S\cap A|=1 :$
\begin{itemize}
\item $S\cap A = T\cap A = \{a_1^{\ell}\}:$
\begin{itemize}
\item $x\in \{b_1^{\ell},\cdots, b_k^{\ell}\} \implies \Delta_f(x|S)=1/2^i+1/2^i$ and $\Delta_f(x|T)=1/2^j+1/2^j$ for $j\ge i$.
\item $x\notin \{b_1^{\ell},\cdots, b_k^{\ell}\} \implies \Delta_f(x|S)=1/2^i$ and $\Delta_f(x|T)=1/2^j$ for $j\ge i$.
\end{itemize}
\item $S\cap A = T\cap A \notin \{a_1^{\ell}\}_{\ell} \implies \Delta_f(x|S) \ge \Delta_f(x|T)$ because of submodularity of $g$.
\end{itemize}
\item if $|S\cap A|=0 \implies \Delta_f(x|T) \le 1/2^{i+1}+1/2^{i+1}$ and $\Delta_f(x|S)= 1/2^j$ for $j\le i$. Thus $\Delta_f(x|S) \ge \Delta_f(x|T)$.
\end{itemize}
\end{itemize} 
Monotonicity is trivial.
\end{proof}

\toRemove{
Also for any subset of $S$ with at least two elements of $A$, $f(S)=2k$. 
For subset $S$ with no element in $A$, if $i=\floor*{\frac{|S|}{k}}$, 
$f(S)$ is defined as 
\[
f(S)= k+k/2+ \dots +(|S|-ik)/2^{i}.
\]
For subset $S$ with exactly one element $a\in A$ such that $a\neq a_1$, if if $i=\floor*{\frac{|S|-1}{k}}$, 
$f(S)$ is defined as 
\[
f(S)= k+ k/2+ \dots +(|S|-1-ik)/2^{i+1}.
\]
Thus if $|S|=k+1$ and it contains exactly one element of $a\in A$ such that $a\neq a_1$ then $f(S)=k+k/2$.
Now suppose $S$  contains $a'$. 
For $S=T$, $f(S)=2k$.  Suppose $S$ contains $k'<k$ elements of $\{b_1, \dots, b_k\}$  and $\ell$ other elements of $B$. 
Let's $t=k'+\ell$, and $i=\floor*{\frac{t}{k}}$, then
\[
f(S)= \min\{2k, k'/2+(k+ k/2+ \dots +(t-ik)/2^{i+1})\}
\]
}
%\scomment{this proof is very vague, especially the claim any algorithm will select $k/2$ of $B$? Phrases like algorithm is not "aware" of something cannot be stated as a fact. You need to prove that the algorithm will not be able to distinguish between the two scenarios. We need to discuss.}



%Let $ {\cal T}^L$ be a collection of (any) $L=n/2k$ sets from $T^\ell, \ell=1,2, \ldots$. W.l.o.g., let's assume ${\cal T}^\ell = \{T_1, \ldots, T_L\}$.   

Denote $B^{\ell} := T^\ell \cap B = \{b_1^{\ell},\cdots, b_k^{\ell}\}$ for $\ell=1,2, \ldots,$. Also, let 
$B'=B\setminus (\bigcup_{\ell=1}^L B^{\ell})$. % where $L:=n/2k$. 
%\scomment{Do you need $T^\ell, \ell =1,\ldots, L$ to be disjoint?} \mcomment{yes}
% $B'=B\setminus (\bigcup_{\ell }^{L} B^{\ell})$ for $L:=n/2k$.
Now define $L$ input instances $\{I_{\ell}\}_{\ell =1,\ldots, L}$, each of size $n$, as follows. For
any arbitrary subset $\tilde{B}\subseteq B'$ of size $n-Lk-1$, 
%\scomment{Which subset $\tilde{B}$? any arbitrary subset?} \mcomment{arbitrary}
define $I_{i}=\bigcup_{\ell=1,\ldots, L}  B^{\ell} \cup \tilde{B} \cup \{a_1^{i}\}$, for  $i=1,\ldots, L$.
%and $I_2=B^1 \cup B^2 \cup \tilde{B} \cup \{a_1^2\}$ (the difference is $a_1^1$ and $a_1^2$).
%Now suppose the input consists of the following:  $T^{\ell}=\{a_1^{\ell}, b_1^{\ell}, \cdots b_k^{\ell} \}$, no other element of $A$ and the remaining elements are from $B':=B\setminus \{b_1^{\ell}, \cdots, b_k^{\ell}\}$. 
Thus the optimal is $T^{\ell}$ for instance $I_{\ell}$, with $f(T^{\ell})=2k$. 
\scomment{$T^\ell$ is of size $k+1$, optimal should be of size $k$. If making $T_\ell$ to be of size $k$ makes it messy, you can initially state that you will consider submodular $k+1$ secretary problem.}


Now consider any algorithm for the submodular \nameSecSL~,and cardinality constraint $k+1$. We denote by $Alg$ the set of $\eta(k+1)$ items selected by the algorithm as part of the shortlist. % (all elements in the shortlist of size $\eta(k)$).
\scomment{We have  used $A$ to denote shortlist in the algorithm. May be you can use a different symbol instead of type $A$ and $B$. }
Let $\bar I$ denote an instance chosen uniformly at random from $I_\ell, \ell=1,\ldots, L$.  
%We choose one of $I_{\ell}$ randomly. \scomment{randomly or arbitrarily?} 
Let $\pi$ denote a random ordering of $n$ items in $\bar I$. 
%We give a random order of $I_{\ell}$, say $\pi$ to the algorithm as input,
%(note that in the secretary problem the elements of input can be selected adversarially but the order should be random).
We denote by random variable $(\bar{I},\pi)$ the randomly ordered input instance to the algorithm. Also we denote by $\bar{T}, \bar{B}$ and $\bar a$, the corresponding $T^{\ell}$, $B^{\ell}$ and $a_1^\ell$.

Now we claim 

%Note that algorithm is not aware of $\ell$.
%Consider an algorithm $Alg$.
%Suppose $a_1^{\ell}$ is the $t$-th elements in the input, and
%elements of input are ordered as $I=(I_1,\cdots, I_n)$.
%Suppose $Alg$ is the set of elements selected by an algorithm.
%Denote by $\bar{B}=\{b_1,\cdots, b_k\}$.

\begin{lemma}
$\mathbb{E}_{(\bar{I},\pi)}[|Alg\cap \bar{B}|] \le k/2+\eta(k+1)/L$.
\end{lemma}
\begin{proof}
Suppose $(e_1,\cdots, e_n)$ indicates the ordered input according to random ordering $\pi$ on $\bar{I}$. %for some $0<\ell<L$.
Now let $t$ be the random variable indicating the index of $a_1^{\ell}$ in $(e_1,\cdots, e_n)$, i.e., $e_t=a_1^{\ell}$. 
%Define $R:=\mathbb{E}[|Alg\cap\{e_1,\cdots,e_{t-1}\}|]$.
Then, due to random ordering, and random choice of $\bar I$ from $I_1, \ldots, I_\ell$, we have
$$\mathbb{E}_{(\bar I, \pi)}[|Alg\cap\{e_1,\cdots,e_{t-1}\}\cap B^1|]= \cdots = \mathbb{E}[|Alg\cap\{e_1,\cdots, e_{t-1}\}\cap B^{L}|]\ .$$
Also, since $B^\ell, \ell=1,\ldots, L$ are disjoint,
$$\sum_{\ell=1}^L \mathbb{E}[|Alg\cap\{e_1,\cdots,e_{t-1}\}\cap B^{\ell}|] \le \eta(k+1)\ .$$
Since $\bar B=B^\ell$ with probability $1/L$,  we have
$$H:=\mathbb{E}[|Alg\cap\{e_1,\cdots, e_{t-1}\}\cap \bar{B}|]=  \frac{1}{L} \sum_{\ell=1}^L \mathbb{E}[|Alg\cap\{e_1,\cdots,e_{t-1}\}\cap B^{\ell}|] \le \frac{1}{L} \eta(k+1)\ . $$ 
%\rightarrow 0$ as $n/\eta(k) \rightarrow \infty$.
Now define
$G:=\mathbb{E}[|Alg\cap\{e_t,\cdots, e_{n}\}\cap \bar{B}|]$.
We have
$$G\le \mathbb{E} [|\bar{B}\cap\{e_t,\cdots, e_n\}|]  \le k/2\ .$$
%Also define $H:=\mathbb{E}[|Alg\cap\{e_1,\cdots,e_{t-1}\cap \bar{B}\}|]$.
%Also, $H\le k-G$.
Thus $$\mathbb{E}[|Alg\cap \bar{B}|] \le G+H\le k/2+\eta(k+1)/L\ .$$
%\rightarrow G$$
%\le k/2$$
%G+(k-G)/2 \le k/2+G/2\le k/2+k/4=3/4k$$.
\end{proof}
Now on input $\bar{I}$, if the algorithm doesn't select $\bar a$, then $f(Alg)\le k+k/2$. Otherwise, if algorithm selects $\bar a$ then 
$$f(Alg)= k+ \frac{1}{2} g(k)+\frac{1}{2} |Alg\cap \bar{B}|$$ therefore $$\mathbb{E}[f(Alg)] \le k+\frac k 2+ \frac k 4+ \frac{\eta(k+1)}{2L} = \frac{7k}{4} + \frac{k\eta(k+1)}{n} \ .$$
%Hence $\mathbb{E}[f(Alg)]  \rightarrow k+k/2+k/4$ as $n\rightarrow \infty$, since $\eta(k)=o(n)$.
Since the optimal is at least $\Ex[f(\bar T)]=2k$, the competitive ratio is upper bounded by
$$ 
%\left(\frac{7k}{4} + \frac{k\eta(k)}{n}\right)\left/\right. 2k = 
\frac{7}{8} + \frac{\eta(k+1)}{2n} = \frac{7}{8} + o(1)\ ,$$
where we used $\eta(k+1)=o(n)$.
\scomment{I think we need to change the upper bound in theorem statement to $7/8 + o(1)$}
%Before arriving $a_1^{\ell}$ algorithm can not distinguish between elements of $B'=\{b_1^{\ell},\dots, b_k^{\ell}\}$
%and the rest of $B$ thus the expected number of elements in $B'$ selected by algorithm before observing $a_1$ goes to $0$ as $n/k\rightarrow \infty$.

%Therefore an online algorithm would select $k/2$ elements of set $B'$ in expectation and also it selects $a_1^{\ell}$ (and $k/2$ other elements from $B\setminus B'$).  Therefore, its $f$ value is $k+k/2+k/4$.
%Hence the competitive ratio is at most $7/8$.


==> bib.tex <==
\bibitem{kleinberg} R. Kleinberg, A Multiple-Choice Secretary Algorithm with Applications to Online Auctions
\bibitem{vondrak} V. Feldman, J. Vondrak, Optimal Bounds on Approximation of Submodular and XOS Functions by Juntas
\bibitem{kleh} T. Kesselheim, A. Tönnis, Submodular Secretary Problems: Cardinality, Matching, and Linear Constraints
\bibitem{mirzasoleiman} A. Badanidiyuru, B. Mirzasoleiman, A. Karbasi, A. Krause, Streaming Submodular Maximization: Massive Data Summarization on the Fly
\bibitem{bateni} M. Bateni, M. Hajiaghayi, M, Zadimoghaddam,  Submodular Secretary Problem and Extensions
%\bibitem{distr} B. Mirzasoleiman, A. Karbasi, R. Sarkar, A. Krause, Distributed Submodular Maximization
\bibitem{recent}  T. Hess, S. Sabato, The monotone submodular secretary problem under a cardinality constraint with limited resources
\bibitem{norouzi} Beyond 1/2-Approximation for Submodular Maximization on Massive Data Streams
\bibitem{linear} B. Mirzasoleiman, A. Badanidiyuru, A Karbasi, J. Vondrak, A. Krause, Lazier Than Lazy Greedy
%\bibitem{swm} M. Kapralov, I. Post, J. Vondrak, Online Submodular Maximization: Beating 1/2 Made Simple
\bibitem{vahab} N. Korula, V. Mirrokni, M. Zadimoghaddam, Online Submodular Welfare Maximization Greedy Beats 1/2 in random order



@article{buchbinder2018online,
  title={Online Submodular Maximization: Beating 1/2 Made Simple},
  author={Buchbinder, Niv and Feldman, Moran and Garg, Mohit},
  journal={arXiv preprint arXiv:1807.05529},
  year={2018}
}


==> conclusion.tex <==
In this paper, we defined a relaxation of the submodular secretary problem with cardinality constraint. We allow the algorithm
to select more than $k$ elements, and the algorithm should output a subset of size $k$ among selected items.
We designed an algorithm with asymptotic
competitive ratio $R$ for any $R<1-1/e$. The total number of selections is only $O(k)$ elements. 
It is open  whether we can generalize this result to more general constraints such as matroid constraints.


==> olderProof.tex <==
\begin{lemma}
\label{lem:piBound}
For any element $i\in S^*$, and $w \in \{1,\ldots, W\}$
\begin{equation}
p_i:=\mathbb{P}(i\in U_w \cup Supp(T_{1,\ldots, w-1}) | T_{1,\ldots, w-1}=T) \ge \frac{\alpha}{k}
\end{equation}
\end{lemma}
\begin{proof}
%Remember that from lemma~\ref{eqprob}, for every configuration $Y \in [k\beta]^n$, we have $\mathbb{P}(Y)=(k\beta)^{-n}$.
%Also from above lemma, for $1\le w\le W$,  $T_{1,\ldots, w}$ and $S_{1, \ldots, w}$ are uniquely defined for each configuration $Y$.
%Suppose $T_{1,\cdots, w-1}=T$ and 
Let $s$ be a slot in the first $w-1$ windows and $s'$ be a slot in window $w$.
If $i\in Supp(T)$ then the statement of the lemma is trivial, so suppose $i\notin Supp(T)$.
By applying Bayes' rule to equation~\ref{eq1} we have
\[
\mathbb{P} (Y_i=s  | T_{1,\ldots, w-1}=T) \frac{ \mathbb{P}(T_{1,\ldots, w-1}=T) }{\mathbb{P}(Y_i=s) } 
\le \mathbb{P} (Y_i=s'  | T_{1,\ldots, w-1}=T) \frac{ \mathbb{P}(T_{1,\ldots, w-1}=T) }{\mathbb{P}(Y_i=s') } 
\]
Also from Lemma~\ref{indep}, $\mathbb{P}(Y_i=s)  = \mathbb{P}(Y_i=s')$ thus 
\[
\mathbb{P} (Y_i=s  | T_{1,\ldots, w-1}=T) 
\le \mathbb{P} (Y_i=s'  | T_{1,\ldots, w-1}=T) 
\]
Furthermore, for slot $s"$ in  windows $w, w+1, \cdots, W$, by applying Bayes' rule to lemma~\ref{afterw}
we have $\mathbb{P} (Y_i=s'  | T_{1,\ldots, w-1}=T) =\mathbb{P} (Y_i=s"  | T_{1,\ldots, w-1}=T)$.
As a result $\mathbb{P}(i \in U_w \cup R_{1,\ldots, w-1} | T_{1,\ldots, w-1}) \ge \frac{\alpha}{k}$.

\end{proof}
%And, for every  $i\in S^*$, define
%\begin{equation}
%p_i :=\mathbb{P}(i\in U_w \cup R_{1,\ldots, w-1} | T_{1,\ldots, w-1})
%\end{equation}
%Then, a corollary of Lemma \ref{lem:piBound} is that $p_i \ge \alpha/k$. 

\begin{lemma}
\label{JIN}
Fix a window $w$. Now, given $U_w, T_{1, \ldots, w-1}$, create $\tilde{S}$ by accepting each item $i\in S^* \cap (U_w \cup R_{1,\ldots, w-1})$ independently with probability $\alpha/(kp_i)$. Then,
the indicator random variables $\{{\mathbf 1}(i\in \tilde S)|T_{1,\ldots, w-1} \}$ for all $i\in S^*$ are independent with  expected value $\alpha/k$.
\end{lemma}
\begin{proof}
Using Lemma \ref{lem:piBound}, the expected value can be derived as
$$\mathbb{P}(i\in \tilde{S}| T_{1, \ldots, w-1}) = \mathbb{P}(i\in \tilde{S}| i\in U_w\cup R_{1,\ldots, w-1},T_{1, \ldots, w-1} )\mathbb{P}(i\in U_w\cup R_{1,\ldots, w-1}| T_{1, \ldots, w-1}) = \alpha/(kp_i) \times p_i = \alpha/k.$$
Next, we show that for any $i,j\in S^*$, random variables ${\mathbf 1}(i\in \tilde S)|T_{1,\ldots, w-1}$ and ${\mathbf 1}(j\in \tilde S)|T_{1,\ldots, w-1}$ are independent. Given the construction of $\tilde S$, it suffices to prove that the random variables ${\mathbf 1}(i\in U_w \cap R_{1,\ldots, w})|T_{1,\ldots, w-1}$ and ${\mathbf 1}(j\in U_w \cap R_{1,\ldots, w})|T_{1,\ldots, w-1}$ are independent. Now, given $T_{1,\ldots, w-1}=T$, if $i \in Supp(T)$ then this is trivial since $R_{1,\ldots, w} =Supp(T)$ so that $\mathbb{P}(i\in U_w \cap R_{1,\ldots, w} | T_{1,\ldots, w-1}=T)=1$. Similarly for $j\in Supp(T)$.

So, assume $i,j  \notin Supp(T)$. Then, the problem reduces to proving that  ${\mathbf 1}(i\in U_w)|T$ and ${\mathbf 1}(j\in U_w)|T$ are independent, i.e., given $T$, $i$ and $j$ will appear in the window $w$ independently. 
To prove this, we show that $\mathbb{P}(Y_i=s|T_{1,\cdots, w-1}=T)=\mathbb{P}(Y_i=s|T_{1,\cdots, w-1}=T \text{ and } Y_j =s')$, i.e., slot assignment of $i$ is independent of the slot assignment of $j$. 

Suppose $Y'$ is a configuration such that $Y'_i=s$ and $Y'_j=s'$, and $T_{1,\cdots, w-1}(Y')=T$. To show the required independence, we show that for every other feasible slot assignment of $j$, there exists a feasible configuration where slot assignment of $i$ is $s$.
More precisely, consider any configuration $Y''$ such that $T_{1,\cdots, w-1} (Y'') =T$ and $Y''_j=s''$ where $s''\ne s'$. (If no such configuration $Y''$ exists, then $Y_j|T$ is always $s'$ so that $s'$ is the only feasible assignment of $j$ given $T$, and the desired statement is trivially true.)
Then by changing $Y_j$ from $s'$ to $s''$ in $Y'$, we can obtain another configuration $\bar{Y}$. In Lemma~\ref{addtoslot}, we show that this change will not effect $T_{1,\cdots, w-1}$, i.e., $T_{1,\cdots, w-1} (\bar Y)=T $. 
Thus configuration $\bar Y$ satisfies the desired statement.
\end{proof}
\scomment{I replaced the proof below with the proof of Lemma 7}
\toRemove{
\begin{proof}
Suppose $i,j \in S^*$. 
If $i \in Supp(T) $ then this is trivial since $\mathbf{1}(i\in \tilde S) | T=1$. \scomment{the preceding statement is not correct, in that case, we just have $p_i=1$.}
So suppose $i,j  \notin Supp(T)$. 
%Now we show that $\mathbb{P}(J_i=1|T_{1,\cdots, w-1}=T)=\mathbb{P}(J_i=1|T_{1,\cdots, w-1}=T \text{ and } J_j =s')$.
Now we show that $\mathbb{P}(Y_i=s|T_{1,\cdots, w-1}=T)=\mathbb{P}(Y_i=s|T_{1,\cdots, w-1}=T \text{ and } Y_j =s')$.
Suppose $Y$ is a configuration in which $Y_i=s$ and $Y_j=s'$, and $T_{1,\cdots, w-1} (Y)=T$.
Also suppose there exists at least one configuration $\bar{Y}$ such that $T_{1,\cdots, w-1} (\bar{Y}) =T$ and $\bar{Y}_j=s"$. \scomment{what if no such configuration exists?}
Then by changing $Y_j$ from $s'$ to $s"$ we obtain a configuration $Y'$. Also from lemma~\ref{addtoslot}, we have  $T_{1,\cdots, w-1} (Y')=T $. 
%It is because in configuration $Y$, $j$ has not been selected in slot $s'$ and its removal will not change $T_{1,\cdots, w-1}$.
%Furthermore since there is a configuration $\bar{Y}$ as described above, adding $j$ to $s"$ will not change $T_{1,\cdots, w-1}$.
Hence the mapping from $Y$ to $Y'$ proves lemma.
\end{proof}
}

\begin{lemma} \label{addtoslot}
Fix a slot $s'$, $T$, $j\notin Supp(T)$. Suppose that there exists  some configuration  $Y'$ such that $T_{1,\cdots, w-1} (Y') =T$ and $Y_j'=s'$. Then, given any configuration $Y''$ with $T_{1,\ldots, w-1}(Y'')=T$, we can replace  $Y''_j$ with $s'$ to obtain a new configuration $\bar Y$ that also satisfies $T_{1,\ldots, w-1}(\bar Y)=T$.
\toRemove{
Suppose there exists at least one configuration $\bar{Y}$ such that   $T_{1,\cdots, w-1} (\bar{Y}) =T$ and $\bar{Y}_j=s$ for $j\notin Supp(T)$.
Then for any configuration $Y$ with  $T_{1,\cdots, w-1} (Y) =T$, by setting $Y_j=s$, we get a new configuration $Y'$
such that $T_{1,\cdots, w-1} (Y') =T$.}
\end{lemma}
\begin{proof}
%Suppose $Y$ is a configuration such that $T_{1,\cdots, w-1} (Y) =T$. 
Suppose the slot $s'$ lies in window $w'$.
If $w' \ge w$ then the statement is trivial. So suppose $w' < w$.
Create an intermediate configuration by {\it removing} the item $j$ from $Y''$, call it $Y^-$. Since $j\notin Supp(T_{1,\cdots, w-1}(Y'')) = Supp(T)$ we have $T_{1,\cdots, w-1} (Y^-) =T$. In fact, for every subsequence $\tau$, the greedy subsequence for $Y''$, will be same as that for $Y^-$, i.e.,   $\gamma_{Y''}(\tau) = \gamma_{Y^-}(\tau)$.
Now add item $j$ to slot $s'$ in $Y^-$, to obtain configuration $\bar Y$. We claim $T_{1,\cdots, w-1} (\bar Y) =T$.
%We only need to show that $j$ will not get selected in slot $s$ in configuration $Y'$.
%Suppose not, then there is a subsequence $\tau$  in the algorithm ending in slot $s$ such that $\gamma_{Y'} (\tau) =\{i_1, \cdots, i_{t-1}, j\}$


By construction of $T_{1,\ldots, w}$, we only need to show that $j$ will not be part of the greedy subsequence $\gamma_{\bar Y}(\tau)$ for any subsequence $\tau, |\tau| = \alpha$ containing the slot $s'$ when the input is in configuration $\bar Y$. To prove by contradiction, suppose that $j$ is part of greedy subesquence for some $\tau$ ending in the slot $s'$. \toRemove{We only need to show that $j$ will not get selected in slot $s$ in configuration $Y'$.
Suppose $j$ gets selected in slot $s$ for some subsequence $\tau$ ending in slot $s$.}
%Thus $\gamma_{Y'}(\tau) = \{i_1, \cdots, i_{t-1}, j\}$. Note that since slots before $s$ are the same as $Y^-$ and $T_{1,\cdots, w-1} (Y^-) =T$, $\gamma_{Y^-}(\tau) = \{i_1, \cdots, i_{t-1}, i_t\}$.
\toRemove{Suppose that $\gamma_{Y^-}(\tau)  := \{i_1, \cdots, i_{t-1}, i_t\} = \gamma_{Y''}(\tau) $.} 
For this $\tau$, let $\gamma_{Y^-}(\tau)  := \{i_1, \cdots, i_{\alpha-1}, i_\alpha\} = \gamma_{Y''}(\tau) $. Note that since the items in the  slots  before $s'$ are identical for $\bar Y$ and $Y^-$, \toRemove{and $T_{1,\cdots, w-1} (Y^-) =T$,} we must have that $\gamma_{\bar Y}(\tau) = \{i_1, \cdots, i_{\alpha-1}, j\}$, i.e.,
$\Delta_f(j | S_{1,\ldots,w'-1} \cup \{i_1,\ldots, i_{\alpha-1}\} ) \ge \Delta_f(i_\alpha | S_{1,\ldots,w'-1} \cup \{i_1,\ldots, i_{\alpha-1}\} ) $.
%$j=\arg \max_{i\in j\cup U_s \cup T_{1, \ldots, w-1}} \Delta_f(i | S_{1,\ldots,w-1} \cup \{i_1,\ldots, i_{t-1}\} \cup \{i\}) $
%$i_t=\arg \max_{i\in U_s \cup T_{1, \ldots, w-1}} \Delta_f(i | S_{1,\ldots,w-1} \cup \{i_1,\ldots, i_{t-1}\} \cup \{i\}) $
On the other hand, since $T_{1,\cdots, w'-1} (Y') = T_{1, \cdots, w'-1}(Y'') = T (\text{restricted to $w'-1$ windows})$,  we have that $\gamma_{Y'} (\tau) =\{i_1, \cdots, i_\alpha\}$.
However, $Y'_j=s'$. Therefore $j$ was not part of the greedy subsequence $\gamma_{Y'}(\tau)$ even though it was in the last slot in $\tau$, implying $\Delta_f(j | S_{1,\ldots,w'-1} \cup \{i_1,\ldots, i_{t-1}\} ) < \Delta_f(i_t | S_{1,\ldots,w'-1} \cup \{i_1,\ldots, i_{t-1}\} ) $. This is  is a contradiction to the earlier observation.


\end{proof}
%Now let  indicator random variable $J_i$ for $i\in S^*$ indicates whether or not $i \in \tilde{S}$ 
%indicates whether or not $e$ appears in $U_w$, i.e., whether or not $U_i^e\in W_{i+1}$.



%Also if $V_e$ is a random variable indicating whether or not $e\in \mathcal{A}$ for $e\in OPT'$,
%we show $\{V_e|Snapshot(i)\}_{e\in OPT'}$ are i.i.d.  with $\mathbb{P}[V_e=1] = \alpha/k$.

%\begin{lemma}
 % %$\mathbb{P}[e=b_j| e\in \mathcal{A}]=1/k$ for $j\in[k]$.
% Random variables $\{V_e|Snapshot(i)\}$,  $ \forall e\in OPT'$ are i.i.d. with $\mathbb{P}[V_e=1]=\alpha/k$.
%\end{lemma}

%\begin{prop}\label{uni}
% Given $i \in \tilde{S}$, we have $\mathbb{P}(i=j)=1/k$, $\forall j\in S^*$.
%\end{prop}

%\scomment{The lemma statement below is not precise- it seems you actually mean uniformly at  random over $\tilde S|T_{1,\ldots, w-1}$, i.e., random also over $U_w$, but given $T_{1, \ldots, w-1}$. We can discuss.}
\begin{prop}\label{uni}
For element $i$ drawn uniformly at random from $\tilde{S}$, we have $\mathbb{P}(i=e)=1/k$, $\forall e\in S^*$.
\end{prop}




Now each element in $\tilde{S}\cap U_w$ has a unique slot in $w$. 
\begin{prop}
Suppose $p_1, \dots, p_{\ell}$ are the slots in $w$ containing at least one element of $\tilde{S}\cap U_w$ (in the same order that they appear in $w$). 
In addition, suppose $b_j\in p_j\cap \tilde{S}$, is the element of $\tilde{S}\cap U_w$ in slot $p_j$ (in case there are more than one element choose one randomly).
%$a_1 ,\cdots, a_t$ are $t$ samples without replacement drawn uniformly at random from $\tilde{S}$.
Then $b_1, \cdots, b_{\ell}$ is a random order of $\{b_1, \cdots, b_{\ell}\}$, and $\{b_1, \cdots, b_{\ell}\}$ are drawn uniformly at random from $\tilde{S}\cap U_w$.
\end{prop}
\scomment{Is Proposition 3 same as saying that $\{Y_i, i\in \tilde S\cap U_w\}$ are i.i.d. and uniformly distributed over slots in $w$? Where is the proof of this proposition?}
\mcomment{Yes, it follows from lemma 7 and the fact that we showed in lemma 6: for slot $s"$ in  windows $w$, by applying Bayes' rule to lemma~\ref{afterw}
we have $\mathbb{P} (Y_i=s'  | T_{1,\ldots, w-1}=T) =\mathbb{P} (Y_i=s"  | T_{1,\ldots, w-1}=T)$.}
%\begin{prop}\label{rord}
%%$a_1 ,\cdots, a_t$ are $t$ samples without replacement drawn uniformly at random from $\tilde{S}$.
%$a_1, \cdots, a_t$ is a random order of $\{a_1, \cdots, a_t\}$, and $\{a_1, \cdots, a_t\}$ are drawn uniformly at random from $\tilde{S}$.
%\end{prop}

On the other hand, elements of $\tilde{S}\cap R_{1,\ldots, w-1}$ 
are not assigned to a  unique slot in $w$ (in the algorithm they were compared against the maximum marginal value in all the slots of $w$).
So we can assign each of them to a unique random slot in $w$.

\begin{prop}
Suppose $q_1, \dots, q_{m}$ are the slots in $w$ assigned to at least one element of $\tilde{S} \cap R_{1,\ldots, w-1}$ (in the same order that they appear in $w$). 
Furthermore, suppose $c_j\in q_j\cap \tilde{S}$, is the element of $\tilde{S}\cap R_{1,\ldots, w-1}$ in slot $q_j$ (in case there are more than one element choose one randomly).
%$a_1 ,\cdots, a_t$ are $t$ samples without replacement drawn uniformly at random from $\tilde{S}$.
Then $c_1, \cdots, c_m$ is a random order of $\{c_1, \cdots, c_m\}$, and $\{c_1, \cdots, c_m\}$ are drawn uniformly at random from $\tilde{S}\cap R_{1,\ldots, w-1} $.
\end{prop}


Now suppose $\{i_1, \cdots, i_t\}=\{p_1, \dots, p_{\ell}\} \cup \{q_1, \dots, q_{m}\}$ (in the same order that they appear in $w$).
From above propositions we have
\begin{prop}\label{rord}
Suppose $a_j \in i_j$  is an element of $i_j \cap (\{p_1, \dots, p_{\ell}\} \cup \{q_1, \dots, q_{m}\})$ (in case there are more than one element choose one randomly).Then
% $a_1, \cdots, a_m$ is a random order of $\{c_1, \cdots, c_m\}$, and $\{c_1, \cdots, c_m\}$ are drawn uniformly at random from $\tilde{S}\cap R_{1,\ldots, w-1} $.
%$a_1 ,\cdots, a_t$ are $t$ samples without replacement drawn uniformly at random from $\tilde{S}$.
$a_1, \cdots, a_t$ is a random order of $\{a_1, \cdots, a_t\}$, and $\{a_1, \cdots, a_t\}$ are drawn uniformly at random from $\tilde{S}$.
\end{prop}





%Consider the set $\mathcal{A}$ we create using the blackbox algorithm. It is a set that we create only for the purpose of argument. Algorithm~\ref{alg:khod} is not aware of this set. 
%Its existence is enough for the algorithm.
The algorithm \textit{guess} the position of elements of $\tilde{S}$, %$OPT\cap W_{i+1}$, 
i.e., slots $i_1, \cdots, i_t$. %, where $t \ge (1-\delta)\alpha$ w.h.p.
In other words, for some $\tau$ in the enumeration of algorithm,  the elements of $\tilde{S}$ lie in the slots of $\tau$. i.e., $\{i_1, \cdots, i_t\} \subseteq \tau$.
%Suppose $a_j\in i_j\cap \tilde{S}$, is the element of $\tilde{S}$ in slot $i_j$.
Suppose $s_j$ is the maximum element selected by the algorithm in $i_j$.
i.e., %$s_j=\omega(\{i_1,\dots,i_j\})$.
$s_j=argmax_{a\in i_j} \Delta_F(a| \gamma{(i_1,\ldots, i_{j-1})})$.
Also let's define $A(j)=\{a_1, \cdots, a_j\} $ and $S(w,j)= S_{1,\ldots, w-1} \cup \{s_1,\cdots, s_j\}$.

\begin{lemma}
%$\mathbb{E}[\Delta_F(S_w | S_{1,\ldots, w-1})] \ge \frac{t}{k} (\frac{k-\alpha}{k}OPT-\mathbb{E}[F(S_{1,\ldots, w-1})])$.
$\mathbb{E}[\Delta_F(s_{j+1}|S(w,j))] \ge \frac{1}{k} (\frac{k-\alpha}{k}OPT-\mathbb{E}[F(S(w,j))])$
\end{lemma}

\begin{proof}
\scomment{What is $OPT'$? What is $P$?}
\mcomment{$P:=S^*\setminus S_{1,\dots, w-1}$, Replaced}
From proposition~\ref{uni} and~\ref{rord}, $a_1$ can be any element in $S^*$, % $OPT\setminus P$, 
w.p. at least $1/k$.
Thus,
\[
\mathbb{E}[\Delta_F(a_1|S_{1,\ldots, w-1}) | T_{1,\ldots, w-1}] \ge \frac{1}{k} \sum_{e\in S^*} \Delta_F(e|S_{1,\ldots, w-1}) %=\frac{1}{k} \sum_{e\in OPT\setminus %P} \Delta_F(e|S_{1,\ldots, w-1}).
\]

%\[
%\mathbb{E}[\Delta_F(a_1|S_{1,\ldots, w-1}) | T_{1,\ldots, w-1}] \ge \frac{1}{k} \sum_{e\in OPT'} \Delta_F(e|S_{1,\ldots, w-1}) =\frac{1}{k} \sum_{e\in OPT\setminus P} \Delta_F(e|S_{1,\ldots, w-1}).
%\]
% (OPT-F(S(i)))$.


Now we use the following well known lemma:
\begin{lemma}%\label{marginalsum}
For any set $A$ and $B$, $\Delta_F(A|B) \le \sum_{a\in A\setminus B} \Delta_F(a|B)$
\end{lemma}
%(Note that in the original version of this lemma the sum is over $A$ instead of $A\setminus B$. But the above format is  stronger if  $A$ and $B$ have intersection. It is the reason we can assign value zero to dummy elements which represent the intersection).
Therefore,
\[
%OPT-F(S(i)) \le \sum_{e\in OPT} \Delta_F(e|S(i)) = \sum_{e\in OPT\setminus P} \Delta_F(e|S(i)) 
OPT-F(S_{1,\ldots, w-1}) \le  \sum_{e\in S^*}  %OPT\setminus P} 
\Delta_F(e|S_{1,\ldots, w-1})  %=  \sum_{e\in OPT'} \Delta_F(e|S(i)) 
\]
Hence,  
\[
\mathbb{E}[\Delta_F(a_1|S_{1,\ldots, w-1})|T_{1,\ldots, w-1}] \ge \frac{1}{k} (OPT-F(S_{1,\ldots, w-1})).
\]
%Now let's define $A(j)=\{a_1, \cdots, a_j\} $ and $S(w,j)= S_{1,\ldots, w-1} \cup \{s_1,\cdots, s_j\}$.
%denote $S(i)\cup \{s_1, \cdots, s_j\} $ by $S(i,j)$. 
Similarly, we can see that 
%$E[\Delta_F(a_{j+1}|S(i,j))] \ge \frac{1}{k} (OPT-F(S(i,j)))$.
\[
\mathbb{E}[\Delta_F(a_{j+1}|S(w,j)) | T_{1,\ldots, w-1}] \ge  \frac{1}{k} \sum_{e\in S^*\setminus A(j)} \Delta_F(e|S(w,j)) 
%=\frac{1}{k} \sum_{e\in OPT\setminus (P\cup A(j))} \Delta_F(e|S(w,j)) 
%\ge \frac{1}{k} \sum_{e\in OPT\setminus (P\cup A)} \Delta_F(e|S(i,j))
\]
Also we have,
\begin{align*} %\label{eq1}
%\begin{split}
%A & = \frac{\pi r^2}{2} \\
% & = \frac{1}{2} \pi r^2
\sum_{e\in S^*\setminus A(j) } %OPT\setminus {(P\cup A(j))}} 
\mathbb{E}[\Delta_F(e|S(w,j)) | T_{1,\ldots, w-1}]  %= \sum_{e\in OPT\setminus P} \Delta_F(e|S(i,j)) 
&\ge \mathbb{E}[F(S^*\setminus A(j)) | T_{1,\ldots, w-1}]-\mathbb{E}[F(S(w,j)) | T_{1,\ldots, w-1}] \\
&\ge \frac{k-\alpha}{k}OPT-\mathbb{E}[F(S(w,j)) | T_{1,\ldots, w-1}] 
%\end{split}
\end{align*}
The last inequality coming from the fact that given $T_{1,\ldots, w-1}$, the set $A(j)$ is a random subset of $S^*$ of size at most  $\alpha$,
so we can apply the following lemma%~\ref{randomsubset}.
\begin{lemma}\label{randomsubset}
For a random subset $A$ of $R$, the expected value of $f(A)$ is at least $\frac{|A|}{k}.f(R)$.
\end{lemma}
Thus 
\[
\mathbb{E}[F(S^*\setminus A(j)) | T_{1,\ldots, w-1}] \ge \frac{k-\alpha}{k}OPT .
\]
Hence, 
\begin{align*}
\mathbb{E}[\Delta_F(s_{j+1}|S(w,j)) | T_{1,\ldots, w-1}] &\ge \mathbb{E}[\Delta_F(a_{j+1}|S(w,j)) | T_{1,\ldots, w-1}] \\
& \ge \frac{1}{k} (\frac{k-\alpha}{k}OPT-\mathbb{E}[F(S(w,j)) | T_{1,\ldots, w-1}]) 
\end{align*}
Now by taking expectation over all possible realizations of $T_{1,\ldots, w-1}$,
\[
\mathbb{E}[\Delta_F(s_{j+1}|S(w,j))] \ge \frac{1}{k} (\frac{k-\alpha}{k}OPT-\mathbb{E}[F(S(w,j))])
\]
%Now by standard techniques we can deduce that $\mathbb{E}[F(S_{1,\ldots, W})] \ge (1-1/e)(\frac{k-\alpha}{k})(1-\delta) OPT$.

 \end{proof}

 
 
Now we prove 
elements of $\tilde{S}$ cover at least  $(1-\delta)\alpha$ slots in $w$, w.h.p. Let $t_w$  denote the number of these slots in $w$.

\begin{theorem}
%Elements of $\tilde{S}$ cover at least  $(1-\delta)\alpha$ slots in $w$, w.h.p.
$(1-\delta)\alpha \le t_w \le (1+\delta)\alpha$, w.h.p. 
\end{theorem}


%Therefore,
%$$\Ex[f(\tilde S \cup S_{1,\ldots, w-1}) - f(S_{1,\ldots, w-1})] \ge \frac{\alpha}{k} f(S^* \cup S_{1,\ldots, w-1}) - f(S_{1,\ldots, w-1}) $$
%INCOMPLETE: the expected size of $\tilde{S}$ is $\alpha$, but the realized size could be larger, and will be truncated to $\alpha$. We need to account for the decrease in objective due to this truncation.
By Chernouf bound, we can show that with high probability each window contains roughly $\alpha$ elements of $\tilde{S}$.

\begin{lemma}\label{bern}
%Suppose $W$ is a $(\alpha,\beta)$ window then
For window $w$
\[
\mathbb{P}(|\tilde{S}| < (1-\delta)\alpha ) %\le exp(-\frac{ (1/2)\alpha^{3/2}}{\alpha+1}) \le exp(-\sqrt{\alpha}/4)
\le \exp(-\delta^2 \alpha/2)
\]
\end{lemma}

Also we can show that roughly $\alpha-2\alpha/\beta$ slots in a window contain at least one element of $\tilde{S}$.

\begin{lemma}\label{slotlemma}
%The probability that one slot has two or more elements is at most $1-e^{-1/\beta}$.
%The fraction of nonempty slots with more than one elements of $OPT$ is at most $\beta(1-e^{1/\beta})$.
%The total number of slots  with more than one element of $OPT$  is at most $2\alpha/\beta$, w.h.p.
Given $|\tilde{S}|=r$,
the total number of slots in $W$ containing at least one element of $\tilde{S}$ is greater than %\alpha-2\alpha/\beta$  w.h.p.
$r(1-r/\alpha \beta)$  w.h.p.
%The total number of elements $e\in OPT\cap W$ such that $Y_e\cap OPT=\{e\}$ is at least $\alpha-2\alpha/\beta$.
%with more than one element of $OPT$  is at most $2\alpha/\beta$, w.h.p.
%$\beta(1-e^{1/\beta})$, w.h.p.
\end{lemma}
\begin{proof}

Suppose $\tilde{S}=\{a_1,\dots, a_r\}$.
%From previous lemma $r\le 2\alpha$, w.p. at least $1-\exp(-\sqrt{\alpha}/3)$.
Let $Z_i$ be a random variable indicating whether or not %$Y_{a_j}\cap OPT\neq \{a_j\}$.
$|Y_{a_j}\cap \{a_1,\dots, a_{j-1}\}| \ge 1$.
%indicating whether $a_k$ is alone in its slot or not.
We have at most $r$ occupied slots, thus the probability that $Z_i=1$ is at most $ r/(\alpha \beta) $ or $\mathbb{E}[Z_i]\le r/\alpha\beta$. Furthermore let $X_i=\sum_{j=1}^{i} Z_j$, then $\mathbb{E}[X_i] \le ri/\alpha\beta$.
%Also let $\mathcal{F}_i$ be the slots elements $1,\cdots, i$  are in, then $L\le \alpha/\beta$. 
Also define the set of filtration $\{\mathcal{F}_i\}$ to be the slots containing elements $\{a_1,\cdots, a_i\}$.
Then $\mathcal{F}_0 \subseteq \dots \subseteq \mathcal{F}_r$.
In addition, $L=\sum_{i\le r}  Var(Z_i|\mathcal{F}_{i-1}) \le r^2/\alpha\beta$.
By Freedman's inequality $\mathbb{P}( X_r > r^2/\alpha\beta + \epsilon )  \le exp(-\frac{\epsilon^2}{4r^2/\alpha\beta +2\epsilon})$.
\end{proof}

Suppose $\delta=1-1/e-R$.
From the above lemmas there are large enough constants $\alpha$ and $\beta$ such that:
\begin{itemize}
\item $r=|OPT\cap W| > (1-\delta/4)\alpha$. Thus $\alpha \ge \frac{1}{\delta^2} \log(1/\delta)$
\item The total number of slots in $W$ containing at least one element of $OPT$ is at least $(1-\delta)\alpha$.
Thus $(1-\delta/4)\alpha(1-(1-\delta/4)/\beta) > (1-\delta)\alpha$.
Therefore $\beta > (1-\delta/4)^2/(3/4\delta) $, so it suffices to have $\beta>\frac{4}{3\delta}$.
\end{itemize}
Hence we choose constants $(\alpha,\beta)$ with $\alpha \ge \frac{8}{\delta^2} \log(1/\delta)$ and $\beta>\frac{4}{3\delta}$,
so that we have above properties.

Therefore $\sum_{w} \min(\alpha, t_w) \ge (1-\delta)k$, w.h.p.
Now by standard techniques we can deduce that 
\begin{theorem}
$\mathbb{E}[F(S_{1,\ldots, W})] \ge (1-1/e)(\frac{k-\alpha}{k})(1-\delta) OPT$.
\end{theorem}

==> saved.tex <==
\noindent {\bf Offline algorithm}
We first present a simpler version of our algorithm which is easier to analyze but not implementable in an online manner. Then, in the next section, we will present an online algorithm which will mimic this offline algorithm very closely.

(Notation: We use shorthand $S_{1,\ldots, w}$ to denote $S_1\cup \cdots \cup S_{w}$.)

\begin{enumerate}
\item Initialize: constants $\alpha \ge 1, \beta \ge 1$ which depend on the constant $\epsilon$.
\item Divide input into $(\alpha, \beta)$ windows.
%Divide into windows and slots: Create $k/\alpha$ `windows'. Assign $n\alpha/k$ candidates to each window uniformly at random, let $U_w$ denote the set of candidates assigned to window $w$ for $w=1,\ldots, k/\alpha$. For each window $w$, create $\alpha\beta$ slots. Assign $\frac n {\beta k}$ out of $\frac {n \alpha} k$candidates to each slot uniformly at random, let $V_{j,w}$ denote the set of candidates assigned to slot $j$ in window $w$ for $j=1,\ldots, \alpha\beta$.
\item Initialize $S_0=\{\}, T_0=\{\}$.
\item For each window $w=1,\ldots, W$:
\begin{itemize}
\item For every $\alpha$-length subsequence $\tau=(s_1,\ldots, s_\alpha)$ of the $\alpha\beta$ slots in window $w$, find a `greedy' sequence $\gamma(\tau)$ of candidates, defined as:
$$\gamma(\tau):=\{i_1, \ldots, i_\alpha\}$$
where
$$i_j := \arg \max_{i\in V_{s_j,w} \cup R_{1,\ldots, w-1}} f(S_{1,\ldots,w-1} \cup \{i_1\ldots, i_{j-1}\} \cup \{i\}) - f(S_{1,\ldots,w-1} \cup \{i_1\ldots, i_{j-1}\})$$
Note that $i_j$ can be picked either from the elements in slot $s_j$ or from $R_1\cup \cdots \cup R_{w-1}$.\\
({\bf To get the online version, primarily we need to use online max algorithm for this step})
\item Set $R_w$ as the union of all the greedy sequences above, i.e., 
$$R_w:=\{\cup_{\tau} \gamma(\tau)\}.$$ 
%where union is taken over all $\alpha$ length subsequences $\tau$ of slots in $w$.
\item Set $S_w$ as the `best' greedy sequence in $R_w$, i.e., $S_w=\gamma(\tau^*)$, where
$$\tau^*:=\arg \max_{\tau} f(S_{1,\ldots,w-1} \cup \gamma(\tau)) - f(S_{1,\ldots,w-1}).$$
\end{itemize}
\item Output $S_{1,\dots, W}$%$A=T_1 \cup \cdots  \cup T_{W}$
\end{enumerate} 
At the end of each window $w$, the above algorithm identifies a set of $\alpha$ `good' elements as the set $S_w$, which as we show later, will satisfy certain approximation properties compared to $\OPT- f(S_{1,\ldots, w-1})$. However, the algorithm actually picks a {\it larger set of elements} $T_w \supseteq R_w$. The set $R_w\backslash S_w$ acts as a buffer which can be used to pick some missed elements later as part of $S_{w'}$ for some window $w'>w$. 

%============================================================

\subsection{Overview and Techniques} 
First we design an asymptotic $1-\epsilon$ algorithm for finding maximum element in a random order input.
%a class of submodular functions that we call them $m$-submodular,
%for any $m>0$. 
The algorithm is very simple. 
It ignores the $\epsilon$-fraction of the input and then selects an item if it improves the current  solution.
We show that with probability $1-\epsilon$ the total number of selections is at most $\log (1/\epsilon)$.
%A special $m$-submodular function for $m=1$ is the function $\max$. 
%As a result we 
In our main algorithm for general monotone submodular functions we  will exploit the fact that we can find maximum marginal value 
of a given submodular function with respect to a subset of items with probability $1-\epsilon$ for $\epsilon>0$.  It requires $\log(1/\epsilon)$ selections.

The main idea of the algorithm is to divide the input into some blocks that we call them $(\alpha,\beta)$ \textit{windows}.
%\begin{definition}
 A \textit{window}, represented by parameters $(\alpha,\beta)$, consists of $\alpha$ consecutive intervals, 
%of length $n/k$. 
each interval is divided into $\beta$ slots. The length of $i$-th slot is a random variable denoted by $X_i$.
Random variables $\{X_i\}$ are coming  from throwing $n$ balls into $k\beta$ bins, $X_i$ would be the number of balls in the $i$-th bin.
%random sample from the binomial distribution $B(n,\frac{1}{k\beta})$.
%of length $\frac{n}{k\beta}$.
%\end{definition}

%It consists of $\alpha$ consecutive intervals, 
%%of length $n/k$. 
%each interval is divided into $\beta$ slots. The length of $i$-th slot is a random variable denoted by $X_i$.
%Random variables $\{X_i\}$ are coming  from throwing $n$ balls into $k\beta$ bins, $X_i$ would be the number of balls in the $i$-th bin.
%%random sample from the binomial distribution $B(n,\frac{1}{k\beta})$.
%%of length $\frac{n}{k\beta}$.
%%Each window consists of smaller subintervals that we call them \textit{slots}.
We apply concentration inequalities for each \textit{window}, and first show that each window  has  roughly $\alpha$ elements of $OPT$, w.h.p., (the probability increases as $\alpha$ increases).
Then we show that the fraction of elements of $OPT$ in a window that lie in different slots is at least $1-1/\beta$.
Therefore by choosing $\beta$ large enough most of them are in different slots.

For each window $w$ the algorithm \textit{guess} the slots in which elements of $OPT\cap w$ lie in. 
By \text{guess} we mean that the algorithm enumerates over all subsets of size $\alpha$ of all $\alpha\beta$  slots in  $w$, and choose 
the one with the maximum marginal gain with respect to previously selected items. (this can be done in an online manner).

In the analysis of the algorithm for each window $w$,
we define an event $T_{1,\cdots, w-1}$ which conditions on the elements that are selected by the algorithm and also the positions in which they get selected by the algorithm. 
By conditioning on $T_{1,\cdots, w-1}$, we prove a lower bound for the expected marginal gain in  window $w$.
Suppose $S_{1,\cdots, w-1}$ is output of algorithm in the first $w$ windows.
The crucial idea is that we show  conditioned on $T_{1,\cdots, w-1}$, elements $e\in OPT\setminus S_{1,\cdots, w-1}$
are more likely to appear in a slot in $w$ than in a slot in windows $1, \cdots, w-1$. 

At the end we have a normalization step in which we make all the elements of $OPT\setminus S_{1,\cdots, w-1}$ to appear with the same probability in $w$. 
Therefore given that one slot in window $w$ contains an element of $OPT$, it can be any of $OPT\setminus S_{1,\cdots, w-1}$ with probability at least $1/k$. Hence the marginal gain for that slot is at least $\frac{1}{k}(OPT-F(S))$. 
We then repeat the argument for all the slots in window $w$  containing elements of the normalized sample.
%==========================================================

\subsection{Online version of the algorithm}

\noindent {\bf Online algorithm}
\begin{enumerate}
\item Initialize: constants $\alpha \ge 1, \beta \ge 1$ which depend on the constant $\epsilon$.
\item Divide into $(\alpha, \beta)$ windows.
%Divide the sequence of candidates into consecutive groups of $\frac{n}{\beta k}$ candidates, referred to as slots (or buckets). And, divide the sequence of slots into consecutive groups of $\alpha \beta$ slots, referred to as {\it windows}.
\item Initialize $S_0=\{\}, T_0=\{\}$.
\item For $w=1,\ldots, W=k/\alpha$:
\begin{itemize}
\item  for every slot $j$ in window $w$
\begin{itemize}
\item Concurrently for all subsequences $\tau\subseteq \{s_1, \ldots, s_{j-1}\}$ with $|\tau|<\alpha$ of slots in $w$, {\bf  run an online max algorithm} on the candidates in $s_j \cup R_{1, \ldots, w-1}$ to identify a set $I(j,\tau)\subseteq s_j \cup R_{1, \ldots, w-1}$ 
of at most  
$\log(1/\delta)$ elements such that the maximum marginal element:
%$$ i_j:=\arg \max_{i\in s_j \cup R_{1, \ldots, w-1}} f(S_{1,\ldots,w-1} \cup \{i_1,\ldots, i_{j-1}\} \cup \{i\}) - f(S_{1,\ldots,w-1} \cup \{i_1,\ldots, i_{j-1}\})$$ 
$$ \arg \max_{i\in s_j \cup R_{1, \ldots, w-1}} f(S_{1,\ldots,w-1} \cup \gamma(\tau)\} \cup \{i\}) - f(S_{1,\ldots,w-1} \cup \gamma(\tau)\})$$ 
lies in $I(j,\tau)$ with probability $1-\delta$. %$1-\frac{\delta}{\alpha{\alpha \beta \choose \alpha}}$. 
Here,
%$$\Gamma(\tau')= \{i_1, \ldots, i_{|\tau'|}\}$$
%with 

%$$i_j:= \max_{i\in I(j, \tau)} f(S_{1,\ldots,w-1} \cup \{i_1, \ldots, i_{j-1}\} \cup \{i\}) - f(S_{1,\ldots,w-1} \cup \{i_1, \ldots, i_{j-1}\})$$
\item {\bf Pick all the candidates in $I(j, \tau) \cap s_j$ for all $\tau$.}
\end{itemize}


\item Let $H_w$ be the union of all the (approximately) greedy sequences above, i.e., 
$$H_w:=\cup_{j\in w, |\tau|\le \alpha} (I(j,\tau)\cap s_j).$$ 
{\bf Note that at the end of window $w$, the candidates picked by the algorithm is $H_1 \cup \cdots \cup H_w$}.
%where union is taken over all $\alpha$ length subsequences $\tau$ of slots in $w$.

\item Set $R_w$ as the union of all the greedy 
%sequences $\tau\subseteq \{s_1, \cdots, s_{\alpha}\}$, i.e., 
$\alpha$-length subsequence $\tau=(s_1,\ldots, s_\alpha)$ of the $\alpha\beta$ slots in window $w$,
$$R_w:=\{\cup_{\tau} \gamma(\tau)\}.$$ 

%\item Set $S_w$ as the `best' subset of size $\alpha$ in $T_w$, i.e., 
%$$S_w:=\arg \max_{S\subseteq T_w, |S|\le \alpha} gf(S_{1,\ldots,w-1} \cup S) - f(S_{1,\ldots,w-1}).$$

\item Set $S_w$ as the `best' greedy sequence in $R_w$, i.e., $S_w=\gamma(\tau^*)$, where
$$\tau^*:=\arg \max_{\tau} f(S_{1,\ldots,w-1} \cup \gamma(\tau)) - f(S_{1,\ldots,w-1}).$$

\end{itemize}
\item Output $S_{1 \cup \cdots W} \cap H_{1,\cdots, W}$
%\item Output $T_1 \cup \cdots \cup T_{k/\alpha}$
\end{enumerate} 
%==========================================================
\subsection{$(\alpha,\beta)$-Windows}

\begin{definition}
Divide the input into $k\beta$ slots. The $i$-th slot, $s_i$, consists of $X_i$ consecutive elements of the input.
Random variables $\{X_i\}$  for $i\in [k\beta]$ are coming  from throwing $n$ balls into $k\beta$ bins, $X_i$ would be the number of balls in the $i$-th bin.
A \textit{window}, represented by parameters $(\alpha,\beta)$, consists of $\alpha \beta$ consecutive slots.
\end{definition}


Note that if the order of the input is $a_1, \dots, a_n$ then the elements inside $s_i$ are $a_{\ell}, a_{\ell+1}, \dots, a_{r}$
where $\ell=X_1+...+X_{i-1}+1$ and  $r=X_1+...+X_i$.




